Improved Implementation of Point Location in General Two-Dimensional Subdivisions

We present a major revamp of the point-location data structure for general two-dimensional subdivisions via randomized incremental construction, implemented in CGAL, the Computational Geometry Algorithms Library. We can now guarantee that the constructed directed acyclic graph G is of linear size and provides logarithmic query time. Via the construction of the Voronoi diagram for a given point set S of size n, this also enables nearest-neighbor queries in guaranteed O(log n) time. Another major innovation is the support of general unbounded subdivisions as well as subdivisions of two-dimensional parametric surfaces such as spheres, tori, cylinders. The implementation is exact, complete, and general, i.e., it can also handle non-linear subdivisions. Like the previous version, the data structure supports modifications of the subdivision, such as insertions and deletions of edges, after the initial preprocessing. A major challenge is to retain the expected O(n log n) preprocessing time while providing the above (deterministic) space and query-time guarantees. We describe an efficient preprocessing algorithm, which explicitly verifies the length L of the longest query path in O(n log n) time. However, instead of using L, our implementation is based on the depth D of G. Although we prove that the worst case ratio of D and L is Theta(n/log n), we conjecture, based on our experimental results, that this solution achieves expected O(n log n) preprocessing time.

==> logn_ratio_table.tex <==
\begin{table}[]
  \begin{center}
    \begin{tabular}{| c | c | c | c |}
    \hline
    Number of Segments 	& $\log(n+1)$ & Depth & Longest query path length \\
    \hline
    15 & 4 & 39 & 15 \\
    \hline
    255 & 8 & 639 & 27 \\
    \hline
    1023 & 10 & 2559 & 33 \\
    \hline
    32767 & 15 & 81919 & 48 \\
    \hline
    $n$ &  &  & $3(log(n+1)+1) $ \\
    \hline
    \end{tabular}
  \end{center}
  \caption{\sf{Depth vs Longest query path length in the $O(\log{n} \div n)$ ratio example (Figure~\ref{fig:depth_vs_log_qlen})}}
\end{table} 

==> sqrt_ratio_table.tex <==
\begin{table}
  \begin{center}
    \begin{tabular}{| c | c | c |}
    \hline
    Number of Segments 	& Depth & Longest query path length \\
    \hline
    225 & 662 & 60 \\
    \hline
    400 & 1182 & 80 \\
    \hline
    10000 & 29902 & 400 \\
    \hline
    $n$ & $3n-\sqrt{n}+2$ & $4*\sqrt{n}$ \\
    \hline
    \end{tabular}
  \end{center}
  \caption{\sf{Depth vs Longest query path length in the $O(\sqrt{n})$ ratio example }}
  \label{tbl:sqrt_ratio_tbl}
\end{table}
%
%%\begin{table}
%  %\begin{center}
%    \begin{tabular*}{0.42\textwidth}{|p{1.5cm}|p{1cm}|p{2cm} |}
%    \hline
%    Number of Segments 	& Depth & Longest query path length \\
%    \hline
%    225 & 662 & 60 \\
%    \hline
%    400 & 1182 & 80 \\
%    \hline
%    10000 & 29902 & 400 \\
%    \hline
%    $n$ & $3n-\sqrt{n}+2$ & $4*\sqrt{n}$ \\
%    \hline
%    \end{tabular*}
%  %\end{center}
%  %\caption{Depth vs Longest query path length in the sqrt ratio example (Figure~\ref{fig:depth_vs_sqrt_qlen})}
%%\end{table} 
